Integrated GIS- and network-based framework for assessing urban critical infrastructure accessibility and resilience: the case of Hurricane Michael

This study presents a framework for assessing urban critical infrastructure resilience during extreme events, such as hurricanes. The approach combines GIS and network analysis with open remote sensing data of the aftermath, vector data on infrastructure, and socio-demographic attributes of populations in affected areas. Using Panama City as an example case study, this paper quantifies hurricane impacts on residents and identifies vulnerable locations for urban planners' attention. Simulations demonstrate how implementing measures at identified weak points can improve system resilience. Comparing pre-hurricane conditions with the aftermath and several years later allows observing network property changes and assessing overall resilience improvements. Findings indicate that individuals over 65 in the studied settlement are more susceptible to disasters, while males in this age category face higher risks.

==> discussion.tex <==
\section{Discussion}
\label{discussion}

The effects of Hurricane Michael on Panama City and its surrounding areas have been profoundly impactful; our study aims to contribute towards understanding these consequences better, with the ultimate goal of informing more resilient transportation networks for future disaster events. Studying the fundamental structure of a network affected by a disaster provides valuable insights into how real-world catastrophes impact measures typically associated with graph robustness and resilience. Our research demonstrates these effects are consistent with existing literature, suggesting their applicability in studying the consequences of hurricanes on road networks specifically. Various effects on network properties during a catastrophic event and its subsequent recovery process were observed. This framework can help identify more vulnerable parts of the network, such as street types, as well as demographic groups that are particularly susceptible to future disasters.

Panama City suffered significant damage from Hurricane Michael, and recovery efforts will take time \cite{wfsu2023}. Living near the coast increases one's vulnerability to natural disasters; people, however, continue to put themselves at risk by living in areas prone to catastrophe inherently inviting trouble by standing in the way of natural disasters. As previously mentioned in the introductory section, there are still many reasons why individuals choose to reside in coastal regions despite their susceptibility to hurricanes and other natural hazards. A notable example, even after being severely damaged by Hurricane Michael, places like Mexico Beach are being repopulated rather than remaining solely as tourist destinations \cite{wfsu2023}.

Usually the challenges encountered arise from the systems people designed \cite{sterman2002}, and the only means by which the susceptibilities of these systems can be reduced is through a deeper comprehension of their nature, followed by improvements in their future design. There are already some instances of moving or abandonment of entire towns located in high-risk disaster areas \cite{guardian2021, cnn2023, bbc2024}. Since mass relocation of affected cities is not feasible, our focus should remain on improving the resilience of these communities. This study has demonstrated that introducing a system-wide improvement to a particularly vulnerable type of street can enhance the overall system's performance. During the preparatory stage, it was noticed that some residential streets were less affected by obstructions caused by Hurricane Michael. Upon closer inspection, these less impacted segments of roads maintained a greater distance from trees (Figure \ref{fig:betterplanning}). This suggests that if this urban design is maintained across the board, another hurricane would result in fewer blocked roadways due to fallen trees. Additionally, planting more robust tree species as suggested by Ward et al. \cite{ward2017} could further improve road resilience.

\begin{figure}[h!]
    \centering
    \includegraphics[width=.54673\textwidth]{graphics/betterresidentialplanning.png}
    \includegraphics[width=.44\textwidth]{graphics/betterresidentialplanning2.png}
    \caption{Examples of improved residential planning involve strategically positioning trees at a secure distance from roadways and buildings to minimize potential harm during disasters. The images illustrate a neighborhood that was less impacted by tree blockage due to maintaining a safe distance for the trees planted away from the roads. Source: \cite{noaa2018}.}
    \label{fig:betterplanning}
\end{figure}

Adding a state related to recovery has taken our research one step closer towards assessing urban resilience dynamics. Future research should explore additional aspects such as urban form considerations and facility placement. Obtaining higher quality data and conducting ground surveys will undoubtedly yield better outcomes. A thorough examination of the destruction caused by a natural disaster would not be possible without access to high-resolution satellite imagery, which is not always available; therefore, it is essential for space agencies and private companies to make these data more accessible. Combining this quantitative approach with qualitative insights from sociological surveys and interviews may present an interesting avenue for further methodological development. The impact of seasonality on tourist visits should also be considered in future studies. Network analysis can be enhanced by introduction of configuration models as the basis for comparison. Comparison to other similar cities unaffected by hurricane will also add to the analysis.

Comparing patterns of various types of catastrophes that damage or obstruct transportation networks and understanding their impact on city resilience is particularly important given the context of climate change and population growth, especially in areas prone to disasters.
